Piquant$\varepsilon$: Private Quantile Estimation in the Two-Server Model

Quantiles are key in distributed analytics, but computing them over sensitive data risks privacy. Local differential privacy (LDP) offers strong protection but lower accuracy than central DP, which assumes a trusted aggregator. Secure multi-party computation (MPC) can bridge this gap, but generic MPC solutions face scalability challenges due to large domains, complex secure operations, and multi-round interactions. We present Piquant$\varepsilon$, a system for privacy-preserving estimation of multiple quantiles in a distributed setting without relying on a trusted server. Piquant$\varepsilon$ operates under the malicious threat model and achieves accuracy of the central DP model. Built on the two-server model, Piquant$\varepsilon$ uses a novel strategy of releasing carefully chosen intermediate statistics, reducing MPC complexity while preserving end-to-end DP. Empirically, Piquant$\varepsilon$ estimates 5 quantiles on 1 million records in under a minute with domain size $10^9$, achieving up to $10^4$-fold higher accuracy than LDP, and up to $\sim 10\times$ faster runtime compared to baselines.

==> macros_IEEE.tex <==
\newif\ifpaper
\papertrue
%\paperfalse


\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother


\usepackage{graphicx} % Required for inserting images
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{amssymb}
%\usepackage{bm}
\usepackage{dsfont}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{capt-of}
\usepackage{nicematrix}
\usepackage{amsmath}
\interdisplaylinepenalty=2500
\makeatletter
\newcommand\setItemnumber[1]{\setcounter{enum\romannumeral\@enumdepth}{\numexpr#1-1\relax}}
\makeatother
%\usepackage{thm-restate}
%\usepackage{algorithm}
%\usepackage{algpseudocode}
%\usepackage{mathtools}
%\usepackage{comment}
%\usepackage{fullpage}
\usepackage{enumitem}
%\usepackage{cancel}
\usepackage{tikz}
%\usepackage{varwidth}
%\usetikzlibrary{trees}
\usepackage[operators,sets]{cryptocode}
\usepackage{tcolorbox, cuted}
\usepackage{subcaption}
%\usepackage[semibold,tt=false]{libertine}
%\usepackage{libertinust1math}
\tcbuselibrary{many}
\tcbset{
    enhanced,
    breakable,
    attach boxed title to top left={
        xshift=0.5cm,
        yshift= -3.5mm, % What do I put here? I'd like to have something like:
%       yshift= -0.5\titleboxheight
    },
    top=4mm,
    coltitle=black,
    beforeafter skip=\baselineskip,
}

\usepackage{comment}

\newenvironment{mybox}[1]{%
    \begin{tcolorbox}[title={#1}, 
    opacityback=1000]%
    }{
    \end{tcolorbox}
}
\newenvironment{mybox2}[1]{%
    \begin{tcolorbox}[title={#1}, 
    colback=white]%
    }{
    \end{tcolorbox}
}


\declaretheorem[name=Theorem, style=plain, numberwithin=section]{theorem}
\declaretheorem[name=Definition, numberwithin=section]{definition}
\declaretheorem[name=Lemma, sibling=theorem]{lemma}
\declaretheorem[name=Fact, sibling=theorem]{fact}
\declaretheorem[name=Corollary, sibling=theorem]{corollary}
\declaretheorem[name=Proposition, sibling=theorem]{proposition}

\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calC{\mathcal{C}}
\def\calD{\mathcal{D}}
\def\calE{\mathcal{E}}
\def\calF{\mathcal{F}}
\def\calG{\mathcal{G}}
\def\calH{\mathcal{H}}
\def\calI{\mathcal{I}}
\def\calJ{\mathcal{J}}
\def\calK{\mathcal{K}}
\def\calL{\mathcal{L}}
\def\calM{\mathcal{M}}
\def\calN{\mathcal{N}}
\def\calO{\mathcal{O}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\calR{\mathcal{R}}
\def\calS{\mathcal{S}}
\def\calT{\mathcal{T}}
\def\calU{\mathcal{U}}
\def\calV{\mathcal{V}}
\def\calW{\mathcal{W}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\calZ{\mathcal{Z}}
\def\E{\mathbb{E}}
\def\R{\mathbb{R}}
\def\Z{\mathbb{Z}}
\def\Frand{\textsf{Rand}}
\def\Fshuffle{\mathcal{F}_\textsf{Shuffle}}
\def\FSort{\mathcal{F}_\textsf{Sort}}
\def\rq{\lfloor qn \rfloor}
\def\XSample{\hat{X}}
\def \d{d}
\def\tA{\tilde{A}}
\def\tB{\tilde{B}}
\def\tC{\tilde{C}}
\def\tD{\tilde{D}}
\def\tE{\tilde{E}}
\def\tF{\tilde{F}}
\def\tG{\tilde{G}}
\def\tH{\tilde{H}}
\def\tI{\tilde{I}}
\def\tJ{\tilde{J}}
\def\tK{\tilde{K}}
\def\tL{\tilde{L}}
\def\tM{\tilde{M}}
\def\tN{\tilde{N}}
\def\tO{\tilde{O}}
\def\tP{\tilde{P}}
\def\tQ{\tilde{Q}}
\def\tR{\tilde{R}}
\def\tS{\tilde{S}}
\def\tT{\tilde{T}}
\def\tU{\tilde{U}}
\def\tV{\tilde{V}}
\def\tW{\tilde{W}}
\def\tX{\tilde{X}}
\def\tY{\tilde{Y}}
\def\tZ{\tilde{Z}}
\def\tf{\tilde{f}}
\def\th{\tilde{h}}
\def\tm{\tilde{m}}
\def\tk{\tilde{k}}
\def\tx{\tilde{x}}
\def\tz{\tilde{z}}


\newcommand{\polylog}{\textnormal{polylog}}
\newcommand{\Lap}{\textnormal{Lap}}

\def\bfx{\mathbf{x}}
\def\bfy{\mathbf{y}}
\def\I{\mathcal{I}}
\def\A{\mathcal{A}}
\def\X{X}
\def \CCb{\textsf{CC}_{\textsf{Bin}}}
\def \CC{\mathsf{CC}}
\def \CCd{\mathsf{CD}}
\def \Xs{X_\mathsf{Sort}}
\def\U{U}
\def\B{D}
\def\R{R}
\def\Q{\mathcal{Q}}
\def\FB{\textsf{FormBuckets}}
\def\SEM{\textsf{SecureExponentialMechanism}}
\def\PS{\textsf{Partial}}
\def\RQ{\textsf{RandomizeQuantiles}}
\def\Pr{\textnormal{Pr}}
\def\FTEM{\mathcal{F}_{\textsf{TEM}}}
\def\FDF{\mathcal{F}_{\textsf{DF}}}
\def\FSample{\mathcal{F}_{\textsf{Sample}}}
\def\Ser{\textsf{S}}
\def\Sim{\textsf{Sim}}
\def\F{\mathcal{F}}
\def\Rec{\textsf{Rec}}
\def\Mult{\textsf{Mult}}
\def\AlgEMSingleQuant{\mathsf{EMSingle}}
\def\Cnt{\textsf{Count}}
\def\FAbs{\mathcal{F}_{\textsf{Abs}}}
\def\Abs{\textsf{Abs}}
\def\Cmp{\textsf{Cmp}}
\def\Equal{\textsf{Equal}}
\def\FLMult{\textsf{FLMult}}
\def\Trunc{\textsf{Trunc}}
\def\Flag{\textsf{Flag}}
\def\Xsam{\X_{\textsf{Sample}}}
\def\XFilter{\X_{F}}
\def\nq{\lfloor q\cdot n \rfloor}
\def\bq{b}
\def\EM{\textsf{EM}}
\def\FSEM{\mathcal{F}_\textsf{SlicingEM}}
\def\FEM{\mathcal{F}_\textsf{EM}}
\def\FBuc{\mathcal{F}_\textsf{Bucketing}}
\def\AQ{\mathsf{AQ}}
\def\Bary{\mathsf{HierMech}}
\def\Shuffle{\mathsf{ShuffleDP}}
\def\LDP{\mathsf{LDP}}
\def\SliceEM{\mathsf{SQ}}
\def\u{u}
\def\rq{r_q}
\def\SEM{\textsf{SlicingEM}}
\def\Buck{\textsf{Bucketing}}
\def \Bu{B}
\def \a{v}
\def \Ans{V}
\def \ad{\blacktriangleright}
\def \TSGD{\textsc{TSGD}}

\def\emd{\textsf{EMD}}
\def\shuffle{\textsf{Shuffle}}

\def\err{\mathsf{err}}
\def\med{\mathsf{med}}
\def\rank{\mathsf{rank}}
\def\nonint{\mathsf{nonint}}
\renewcommand{\RR}[1]{\mathsf{RR}_{#1}}
\renewcommand{\epsilon}{\varepsilon}
\def\name{\textsf{Piquant$\epsilon$}}

\newcommand{\arc}[1]{\textcolor{purple}{ARC: #1}}
\newcommand{\fb}[1]{\textcolor{red}{FB: #1}}
\newcommand{\anders}[1]{\textcolor{orange}{[Anders: #1]}}
\newcommand{\ji}[1]{\textcolor{green}{[Jacob: #1]}}
\newcommand{\hk}[1]{\textcolor{blue}{Hannah: #1}}
\newcommand{\rp}[1]{\textcolor{magenta}{Rasmus: #1}}

 \newcommand{\squishlist}{
	\begin{enumerate}[label=\arabic*.]
		{
			\setlength{\itemsep}{0pt}
			\setlength{\parsep}{0.5pt}
			\setlength{\topsep}{0.5pt}
			\setlength{\partopsep}{0pt}
			\setlength{\leftmargin}{1em}
			\setlength{\labelwidth}{1em}
			\setlength{\labelsep}{0.5em} } }
	
\newcommand{\squishend}{
\end{enumerate}  }

\newcommand{\squishl}{
	\begin{list}
    {$\bullet$}
		{
			\setlength{\itemsep}{0pt}
			\setlength{\parsep}{0.5pt}
			\setlength{\topsep}{0.5pt}
			\setlength{\partopsep}{0pt}
			\setlength{\leftmargin}{1em}
			\setlength{\labelwidth}{1em}
			\setlength{\labelsep}{0.5em} } }
	
\newcommand{\squishe}{
\end{list}  }



